SCLib: A Practical and Lightweight Defense against Component Hijacking in Android Applications

Cross-app collaboration via inter-component communication is a fundamental mechanism on Android. Although it brings the benefits such as functionality reuse and data sharing, a threat called component hijacking is also introduced. By hijacking a vulnerable component in victim apps, an attack app can escalate its privilege for operations originally prohibited. Many prior studies have been performed to understand and mitigate this issue, but no defense is being deployed in the wild, largely due to the deployment difficulties and performance concerns. In this paper we present SCLib, a secure component library that performs in-app mandatory access control on behalf of app components. It does not require firmware modification or app repackaging as in previous works. The library-based nature also makes SCLib more accessible to app developers, and enables them produce secure components in the first place over fragmented Android devices. As a proof of concept, we design six mandatory policies and overcome unique implementation challenges to mitigate attacks originated from both system weaknesses and common developer mistakes. Our evaluation using ten high-profile open source apps shows that SCLib can protect their 35 risky components with negligible code footprint (less than 0.3% stub code) and nearly no slowdown to normal intra-app communications. The worst-case performance overhead to stop attacks is about 5%.

==> backg.tex <==
\section{Preliminaries}
\label{sec:backg}


\input{model}


\input{current}


==> current.tex <==
\subsection{Current State of Component Hijacking Risks in the Wild}
\label{sec:current}


Can refer to MoST'16 paper, and also our own survey.


More recent Android system issues


==> implement.tex <==
%\section{Implementing A \name Prototype}
\section{Implementation}
\label{sec:implement}


We have implemented a proof-of-concept \name prototype for all four types of Android components.
It consists of 567 lines of Java codes, which we try to keep short.
It implements all the policies we have designed in Table~\ref{tab:macpolicy}, and could be easily extended to support more.
Additionally, we write 313 lines of Python codes to identify risky components in the compiling-time phase.


Among a number of engineering issues we have solved during the implementation, we identify and overcome three major challenges, as shown in the following sections.
%TODO
These challenges appear because of the uniqueness of the \name approach.
Addressing them also brings broader implications for other app-layer access control defenses.  



\subsection{Recovering Caller Identity via the Binder Side Channel}
\label{sec:implementCaller}



\begin{figure}[t!]
%\vspace{-2ex}
\begin{adjustbox}{center}
\includegraphics[width=0.48\textwidth]{binderLog}
\end{adjustbox}
%\vspace{-4ex}
\caption{\small An example of the Binder \texttt{transaction\_log}.}
\label{fig:binderlog}
%\vspace{-4ex}
\end{figure}


As previously mentioned in \mysec\ref{sec:primitive}, Android currently fails to provide the caller identity information to most of callee components, because the \texttt{Binder.getCallingUID()} API cannot work properly in non-Binder threads.
Note that most of entry functions in Table~\ref{tab:entryfuncs} do not run in the Binder threads.
Moreover, since \name cannot modify Android source codes, we require an app-layer solution to address this limitation.
This poses a unique challenge beyond the existing system-level technique like Scippa~\cite{Scippa14}.  


Our solution is to leverage the Binder side channel at the path of \texttt{/sys/kernel/debug/binder/transaction\_log}.
More specifically, for each intercepted IPC call, we retrieve the recent Binder logs from this side channel and analyze them to recover the corresponding caller app identity.
\myfig~\ref{fig:binderlog} shows a \texttt{transaction\_log} example when an attack app exploits an \texttt{Activity} component in the victim app.
Each Binder log starts with a unique transaction id, followed by the Binder action and the process/thread ids of the caller and callee processes. 
The last part, node information, is not important so we skip here.
In the Binder level, app processes do not directly interact with each other.
Instead, the high-level IPC always involves a number of the interaction between apps and system processes (see~\cite{Scippa14} for more details).
For example, the attack app (PID: 7569) and the victim app (PID: 6767) here leverage the \texttt{surfaceflinger} and \texttt{system\_server} processes to delegate their communication.


Our extensive tests of Binder logs in different components show that they all follow the same pattern, based on which, we propose a simple algorithm to recover caller identities.
We still use \myfig~\ref{fig:binderlog} to illustrate this algorithm.
The first step is to locate the Binder log that ``calls from'' the callee PID for the first time, i.e., the transaction 177345 in the figure.
Then we trace back to identify the first app process, i.e., PID 7569 here, which is the caller app we are looking for.
Since there is no fixed PID patten for non-system processes, we further extract the corresponding UID and package name for analysis.
More specifically, if the UID is lower than 10000 or if the package name is a system binary, it must be a system process. 


Since there is a timing window to retrieve the recent Binder logs, \name performs the Binder analysis before other modules.
Moreover, we focus on saving logs first and delay the real analysis afterwards.
Our tests confirm that we can stably retrieve the required Binder logs.
Additionally, SEAndroid on certain modern devices may not allow a regular app to read the Binder logs.
However, this is device-specific, as documented by Google~\cite{DevicePolicy}.
As an example, the Nexus 4 phone (with Android 5.0) allows even in the enforcing mode.





\subsection{Extracting Component Attributes by Runtime Manifest Analysis}
\label{sec:implementAttr}

The second challenge is to extract component attributes that are lack of API support, as introduced in \mysec\ref{sec:primitive}.
\name therefore performs Android manifest analysis by itself.
In particular, we choose the runtime analysis instead of the offline analysis, because it does not bother developers and neither needs the additional file storage.
Also, it is immune to app updates and can handle new components well.


The basic procedure of manifest analysis is to retrieve the whole \texttt{AndroidManifest.xml} file of the callee app and do parsing.
Specifically, for the callee component, we extract its raw ``exported'' status, the registered Intent actions, and the associated permissions.
Further, we correlate the app permission entries to obtain their protection levels and see whether an associated permission is defined by the system or the callee.
Moreover, we build a list of system-defined and system-only Intent actions based on the Stowaway result~\cite{Stowaway11} and Android source codes, so that we can determine whether a given component listens to system Intent actions.





\subsection{Popping Up Alerts via the Dialog-like Activity Transition}
\label{sec:implementUI}

To enforce the ``alert'' policies, \name needs to pop up alert boxes for users to choose ``allow'' or ``deny''.
However, this is a challenging task due to the following reasons:
\begin{itemize}
\item Background components such as \texttt{Provider} and \texttt{Service} do not have an appropriate UI \texttt{Context} to display the alert box dialog.
In particular, \texttt{Provider} retrieves the caller app's \texttt{Context} object instead of the callee app's~\cite{Context}, and it is forbidden to display one app's UI elements using another app's \texttt{Context}.
Even for \texttt{Activity}, it cannot pop up dialogs when \texttt{onCreate()} is still being intercepted (i.e., not return yet).

\item Some components' entry functions (e.g., \texttt{Activity}'s \texttt{onCreate()} and \texttt{Receiver}'s \texttt{onReceive()}) require to return in a short time.
Therefore, we cannot hold on the execution of these functions and wait for users' decisions.
\end{itemize}


To address these issues, we opt to a different strategy instead of directly displaying an alert box.
The basic idea is to launch a dialog-like \texttt{Activity} from the intercepted component via the \texttt{startActivity()} API.
For entry functions that are sensitive to the execution time, \name immediately returns the execution flow to them by assuming users choose the ``deny''. 
If later users select the ``allow'', \name further re-sends the same Intent content\footnote{\small \texttt{Provider}'s entry functions are not sensitive to to the execution time, so we focus on the Intent-based communication here.} on behalf of the original caller app.
Since the callee app has no way to distinguish the caller identity, the original execution flow can resume.
%TODO startActivityForResult; and Service's bindService()
For other time-insensitive entry functions, \name pauses their component execution and wait for users to make a decision on the alert box (within the timeout value). 


To implement this dialog-like Activity transition approach, we identify and handle the following details:
\begin{compactitem}
\item To enable background components be able to launch the alert Activity, we set a special \texttt{Intent} flag called \texttt{FLAG\_ACTIVITY\_NEW\_TASK}.

\item After users click alert box buttons, we automatically return to the original UI state, which is important for maintaining a good user experience. We set one more \texttt{Intent} flag called \texttt{FLAG\_ACTIVITY\_MULTIPLE\_TASK} so that our alert Activity can naturally go back to the previous UI state after calling the \texttt{Activity.finish()} API.

\item To avoid alert boxes appear in the history of recent \texttt{Activity} components, we further set the third \texttt{Intent} flag called \texttt{FLAG\_ACTIVITY\_EXCLUDE\_FROM\_RECENTS}.

\item To pause the component execution and wait for user decisions, \name initializes a lock object and sets this object into the ``wait'' status after invoking the \texttt{startActivity()} API. Once users click the buttons, the alert Activity will notify the ``waited'' lock object to be released. Then, the lock object will no longer wait and the paused component will resume its execution. To avoid the unnecessary long-time waiting, we set a timeout value, 30 seconds in our prototype.

%TODO
%\item \red{TODO}
\end{compactitem}


==> seclib.tex <==
\section{\name: Secure Component Library}
\label{sec:seclib}




%\subsection{A Real-world Example}
%\label{sec:example}
%
%Use the Terminal Emulator's code example\ldots




\subsection{Design Overview}
\label{sec:overview}


\myfig~\ref{fig:seclib} presents the overall design of \name.
In the high-level view, \name is a regular user-space library that could be easily integrated into apps on different Android platforms.
\name aims to be a secure component library that performs in-app mandatory access control (MAC) on behalf of app components to defend against component hijacking.
With a set of pre-defined MAC policies in \name, developers no longer need to worry about the by-default system weaknesses or common developer mistakes.
Moreover, due to the library-based nature, \name inherently requires \textit{no} firmware modification or app repackaging (O1:~\gou; O2:~\gou).


\begin{figure}[t!]
%\vspace{-2ex}
\begin{adjustbox}{center}
\includegraphics[width=0.4\textwidth]{scliboverall}
\end{adjustbox}
%\vspace{-5ex}
\caption{\small The design overview of \name.}
\label{fig:seclib}
%\vspace{-4ex}
\end{figure}


\begin{table*}[t!]
%\vspace{-2ex}
\centering
\caption{\scriptsize Component entry functions that need to be intercepted, characterized by component types and IPC caller APIs.}
\scalebox{1.1}{
\begin{threeparttable}
%\rowcolors{1}{mygreen}{}
\begin{tabu}{ |c | c | l|}

\hline
\rowfont{\bfseries}
\rowcolor{LightGray}
Component types & IPC caller APIs\tnote{\dag} & Interested entry functions\tnote{\dag} of IPC callee components \tabularnewline
\hline
\hline

\multirow{2}{*}{\texttt{Activity}~\cite{Activity}} & \texttt{Context}\cite{Context}\texttt{.startActivity()} & \multirow{2}{*}{\texttt{onCreate(Bundle)}; \texttt{onStart()}; \texttt{onNewIntent(Intent)}}\tabularnewline
& \texttt{Activity.startActivityForResult()} & \tabularnewline
\hline

\multirow{2}{*}{\texttt{Service}~\cite{Service}} & \texttt{Context.startService()} & \texttt{onCreate()}; \texttt{onStartCommand()}\tnote{\ddag} ; \texttt{onHandleIntent(Intent)} \tabularnewline
& \texttt{Context.bindService()} & \texttt{onCreate()}; \texttt{onBind(Intent)}; \texttt{onRebind(Intent)} \tabularnewline
\hline

\multirow{2}{*}{\texttt{Receiver}~\cite{BroadcastReceiver}} & \texttt{Context.sendBroadcast()} & \multirow{2}{*}{\texttt{onReceive(Context, Intent)}} \tabularnewline
& \texttt{Context.sendOrderedBroadcast()} & \tabularnewline
\hline

\multirow{6}{*}{\texttt{Provider}~\cite{ContentProvider}} & \texttt{ContentResolver}\cite{ContentResolver}\texttt{.query()}  & \texttt{query(Uri, String[], String, String[], String)} \tabularnewline
& \texttt{ContentResolver.insert()}  & \texttt{insert(Uri, ContentValues)} \tabularnewline
& \texttt{ContentResolver.bulkInsert()}  & \texttt{bulkInsert(Uri, ContentValues[])} \tabularnewline
& \texttt{ContentResolver.update()} & \texttt{update(Uri, ContentValues, String, String[])} \tabularnewline
& \texttt{ContentResolver.delete()}  & \texttt{delete(Uri, String, String[])} \tabularnewline
& \texttt{ContentResolver.openFileDescriptor()}  & \texttt{openFile(Uri, String)} \tabularnewline
\hline

\end{tabu}
\begin{tablenotes}
%\footnotesize
\item[\dag] For simplicity, we skip the parameters of caller APIs and the class names of entry functions.
\item[\ddag] An old-SDK version of \texttt{onStartCommand(Intent, int, int)} is \texttt{onStart(Intent, int)}, which should be also covered.
\end{tablenotes}
\end{threeparttable}
}
\label{tab:entryfuncs}
%\vspace{-2ex}
\end{table*}


\name is a lightweight defense by design in its both phases, i.e., the offline and the runtime phases in \myfig~\ref{fig:seclib}.
In the offline phase, we design \name to first identify risky components that need protection, so that not all (exported) components' performance would be affected.
To intercept incoming IPC flows, we add only limited amounts of stub codes into each entry function of risky components (usually two lines of codes per entry).
In this way, the code footprint introduced by \name is also minimized.
Further, in the runtime phase, we collect enforcement primitives and enforce policy checking only at entry points.
All these design choices make \name lightweight (O4:~\gou).


With \name, the incoming IPC flow no longer directly executes the component codes. 
Instead, it has to first go through \name's checking with three possible outputs: \texttt{deny}, \texttt{alert}, and \texttt{allow}.
Only in the \texttt{allow} case, the execution flow then goes back to the component codes.
While for the \texttt{alert} case, \name pops up an alert box for users to make a further decision.
Only when he or she allows, the flow would then resume.
To make practical in-app policies to facilitate the access control, \name collects a number of enforcement primitives that previous efforts have not fully leveraged and takes all four types of Android components into consideration (O3:~\gou).




\subsection{Identifying Risky Components}
\label{sec:risky}

It is difficult to define the concept of ``risky'' because it is one of the salient features that apps can communicate with each other's exported components via inter-component communications. On one hand, exported components are potentially risky, however, not all exported components should be restrained from being accessed. For example, the main activity of an app is supposed to be exported at all time.
On the other hand, it depends on the developers' configuration whether an app component is exported. Unfortunately, there has been misconfiguration during the development. 

We identify risky components in a conservative manner. 
We take into consideration both the characteristics of different components and the possible misconfiguration of developers. We use the following rules to identify risky components that need to be protected. 1) For \texttt{Activity}, if there is any customized actions string in an activity's intent-filters, we consider it is risky.
2) For \texttt{Provider}, if there is no explicit attribute configuring it as exported, we consider it is risky. 3) For \texttt{Service} and \texttt{Receiver}, if the component is implicitly exported, we consider it risky.
We show the core idea of this process in pseudocode in Algorithm~\ref{alg:Risky Component Identification.}.


\begin{algorithm}
\caption{Risky Component Identification.}
\label{alg:Risky Component Identification.}
\begin{algorithmic}[1]
\footnotesize
\Require 
\Statex $t$: the component type;
\Statex $attr$: the raw ``exported'' attribute; It can be $true$, $false$, or $null$ if the component does not claim this attribute.
\Statex $expt$: whether the component eventually exports or not;
\Statex $ca$: whether the component registers custom actions.
\Ensure $risky$: whether the component is risky or not.
\Procedure{RiskyComponent}{$t$, $attr$, $expt$, $ca$}
 \State $risky \gets false$ 
 \If{$t$ = \texttt{Activity}}
 	\If{$expt$ = $true$ and $ca$ = $true$}
 		\State $risky \gets true$
 	\EndIf
 \EndIf
 \If{$t$ = \texttt{Provider}}
 	\If{$attr$ != $false$}
 		\State $risky \gets true$
 	\EndIf
 \EndIf
 \If{$t$ = \texttt{Service} or $t$ = \texttt{Receiver}}
 	\If{$attr$ = $null$ and $expt$ = $true$}
 		\State $risky \gets true$
 	\EndIf
 \EndIf
 \State return $risky$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Adding Stub Codes in Entry Functions}
\label{sec:instrumententry}


To route incoming IPC flows to \name for access control, we add stub codes into entry functions of risky components.
Table~\ref{tab:entryfuncs} characterizes the component entry functions that need to be intercepted.
They are organized by different component types and IPC call APIs.
A detailed explanation on these entry functions is available in the Appendix.


After locating entry functions, we perform code instrumentation to insert \name's stub codes.
The real implementation of these stub codes are referred to \name's four static Java classes, namely \texttt{SecActivity}, \texttt{SecService}, \texttt{SecReceiver}, and \texttt{SecProvider}.
We identify three kinds of \name instrumentation:


\lstinputlisting[
float=t!,
style=customJava,
basicstyle=\ttfamily\scriptsize,
label={lst:entryreceiver},
caption={\small Instrumenting \texttt{Receiver}'s \texttt{onReceive}.}
]{entryreceiver.java}

\lstinputlisting[
float=t!,
style=customJava,
basicstyle=\ttfamily\scriptsize,
label={lst:entryprovider},
caption={\small Instrumenting \texttt{Provider}'s \texttt{query}, with the additional \texttt{this} variable.}
]{entryprovider.java}

\lstinputlisting[
float=t!,
style=customJava,
basicstyle=\ttfamily\scriptsize,
label={lst:entryactivity},
caption={\small Instrumenting \texttt{Activity}'s \texttt{onCreate}, with the additional \texttt{getIntent()} and \texttt{finish()} API calls.}
]{entryactivity.java}


\begin{enumerate}
\item \textbf{Basic instrumentation:}
Most of \name instrumentation just add two lines of codes in the prologue of entry functions.
They intercept original entry parameters and a few context parameters to \name.
Listing~\ref{lst:entryreceiver} shows the example of instrumenting \texttt{Receiver}'s \texttt{onReceive}.
It simply delivers the original \texttt{Context} and \texttt{Intent} parameters to \texttt{SecReceiver}'s \texttt{receive} function for access control (line 2).
If the access is not allowed by policies, the stub code returns without giving the control flow back to original code (line 3).
In most cases, we need to intercept additional parameters such as component \texttt{Context}, from which \name then can extract enforcement primitives.
To obtain the \texttt{Context}, we deliver a \texttt{this} variable to the stub code.
Listing~\ref{lst:entryprovider} illustrates such an example for \texttt{Provider}.

\item \textbf{Special instrumentation for \texttt{Activity}:}
As shown in Listing~\ref{lst:entryactivity}, there are two differences for the stub code in \texttt{Activity}'s entry functions.
First, it should be put after the parent function in line 2.
Otherwise, the \texttt{SuperNotCalledException} will occur.
Second, we need to additionally call the \texttt{finish()} API to recycle user interface is access is denied.
Moreover, we invoke the \texttt{getIntent()} API to explicitly obtain the Intent value.

\item \textbf{Special instrumentation for bound services:}
As explained in the Appendix, we shall treat Binder interface functions as individual entries.
Therefore, for a bound \texttt{Service} such as the RemoteService~\cite{AIDL} in Listing~\ref{lst:entryservice}, we instrument not only its \texttt{onBind} as usual, but also the \texttt{getPid} function in a way similar to how we instrument \texttt{Provider}'s entries.
That is, we record both the interface name (``getPid'') and all its parameters (\texttt{null} in this case).
\end{enumerate}


\lstinputlisting[
float=t!,
style=customJava,
basicstyle=\ttfamily\scriptsize,
label={lst:entryservice},
caption={\small The special instrumentation for a bound \texttt{Service} named RemoteService~\cite{AIDL}. \name instruments \texttt{onBind} as usual, and further instruments Binder interface functions (\texttt{getPid} here) as for \texttt{Provider}'s entries.}
]{entryservice.java}


%\begin{enumerate}
%\item \textbf{Instrumentation with original parameters:}
%This kind of instrumentation delivers original entry parameters to \name for decision making.
%An example is to instrument \texttt{BroadcastReceiver}'s \texttt{onReceive}, as shown in Listing~\ref{lst:entryreceiver}.
%The original \texttt{Context} and \texttt{Intent} parameters are delivered to \texttt{SecReceiver}'s \texttt{receive} function for access control (line 2).
%If the access is not allowed by policies, the instrumentation code simply returns without giving the control flow back to original code (line 3).
%
%\item \textbf{Instrumentation with additional parameters:}
%Quite often, the \entryAC instrumentation needs to intercept additional parameters.
%A representative example is the component \texttt{Context} variable, from which \name only then can extract component identity and attribute for policy enforcement.
%To obtain the \texttt{Context}, we simply deliver a \texttt{this} variable to \name's instrumentation code.
%Listing~\ref{lst:entryprovider} shows an example for \texttt{SecProvider} to retrieve the \texttt{Context} via the \texttt{this} variable (line 2).
%
%\item \textbf{Instrumentation with \texttt{getIntent()}:}
%A special class of the second kind of instrumentation is to intercept the incoming \texttt{Intent} for \texttt{Activity}.
%Both \texttt{onCreate} and \texttt{onStart} have no access to \texttt{Intent} in their parameters.
%Instead, \texttt{SecActivity} needs to invoke the \texttt{getIntent()} API to explicitly obtain the \texttt{Intent} value for these two entries.
%
%\item \textbf{Instrumentation for bound services:}
%\end{enumerate}




\subsection{Extracting Enforcement Primitives}
\label{sec:primitive}

At runtime, \name automatically collects a set of valuable enforcement primitives that have not been fully leveraged in previous works, including caller and callee app identities, various component attributes, and input data of incoming requests.
 

\textbf{App identity.}
We extract the identity information of both caller and callee apps for policy making.
%TODO where to define UID
We use the package name (e.g., \texttt{com.whatsapp} for WhatsApp) instead of the app UID to represent an app identity, because some apps (e.g., Chrome) may have multiple UIDs.
We further combine app signatures to determine whether two apps are from the same developer.
In this paper, we uniformly denote these identity information by $Id_a$ and $Id_v$, which represent the caller and the callee identity, respectively.
Then, $Id_a \neq Id_v$ represents that an incoming IPC request is from an external app.


Obtaining the callee identity is simple, because there are mature APIs for this purpose.
For example, we can retrieve the callee app package name from \texttt{ApplicationInfo}, a data structure returned from the \texttt{Context.getApplicationInfo()} API.
However, it is challenging to extract the caller identity.
Although there is an API called \texttt{Binder.getCallingUID()}, it currently fails to provide the caller identity information to most of callee components, except \texttt{Provider} and \texttt{Service}'s Binder interface functions.
As explained in~\cite{Scippa14}, this is because most components' entry functions do not run inside the Binder thread, only in which the \texttt{getCallingUID()} API can work properly.
Further, as an app-layer defense, \name cannot modify Android source codes as Scippa~\cite{Scippa14} to address this limitation.
%This then sounds like an impossible mission. 
Fortunately, after researching several potential workarounds, we eventually find a Binder side channel that can help recover caller app identities at the application layer.
We will present the details in \mysec\ref{sec:implementCaller}.


\textbf{Component attribute.}
We further extract a variety of component attributes to facilitate access control.
These component attributes are claimed by Android apps in their manifest files, i.e., \texttt{AndroidManifest.xml}.
We denote each attribute by $XxxAttr$, such as $ExportedAttr$ for the ``exported'' attribute, $PermAttr$ for the permission attribute, and $ActionAttr$ for the \texttt{Intent} actions registered by components.
Additionally, there are a number of system-defined permissions and actions, which we denote by $SysPerms$ and $SysActions$, respectively.
A list of such permissions and actions are available in~\cite{SysPerms, SysActions}.
Among them, if one permission can be only used by system or an action can be only sent by system, we further denote them by $SysOnlyPerm$ and $SysOnlyAction$, respectively.


Most of component attributes can be directly retrieved through existing APIs, e.g., those defined in the \texttt{ComponentInfo} class and its subclasses (\texttt{ActivityInfo}, \texttt{ProviderInfo}, and \texttt{ServiceInfo}).
But we also find that certain attributes, notably $ExportedAttr$ and $ActionAttr$, are lack of robust or convenient APIs. 
For example, although there is an \texttt{exported} field in the \texttt{ComponentInfo} class, it does not tell whether the component is explicitly or implicitly exported\footnote{\small A component is implicitly exported when it does not claim the \texttt{exported=true} but automatically exported by Android according to some by-default rules (e.g., registering the \texttt{intent-filter} for Intent-based components and \texttt{Provider} before Android 4.2). More details are available in~\cite{ComDroid11} and official Android documents.}.
Instead, it simply reports \texttt{true} for the exported case, no matter the component explicitly defines the ``exported'' attribute or not.
To obtain the raw $ExportedAttr$, \name has to perform runtime manifest analysis by itself, as we will present in \mysec\ref{sec:implementAttr}.
 

\textbf{Input data of incoming IPC requests.}
Another important primitives we collect are the input data of incoming IPC requests.
Some inputs may contain maliciously crafted data (so we can make corresponding policies to stop them), while most of them provide fine-grained information to help users make access control decisions on alert boxes.
As a prominent example, the \texttt{Intent} input could contain the \texttt{action}, the data \texttt{Uri}, the \texttt{category}, and a couple of extra key-value mappings.
\name iterates the whole \texttt{Intent} structure and presents them to users if necessary.
Similarly, for \texttt{Provider} components, we leverage the stub codes in Listing~\ref{lst:entryprovider} to obtain the whole input parameters, including the data \texttt{Uri} and the \texttt{projection} value. 


To refer to these input data in our policies, we denote each input value by $InputXxx$.
For example, the incoming \texttt{Intent} action is represented as $InputAction$, the data \texttt{Uri} is denoted by $InputUri$, and so on.




\subsection{Enforcing In-App Access Control}
\label{sec:policy}


\begin{table*}[ht!]
%\vspace{-2ex}
\centering
\caption{\small MAC policies in \name. Here we list six representative policies (P1 to P6) we have designed.}
\scalebox{1.08}{
\begin{threeparttable}
\begin{tabu}{ |c | l | c | l | c|}

\hline
\rowfont{\bfseries}
\rowcolor{LightGray}
ID & Policy Name & \dag & Policy Representation & \ddag \tabularnewline
\hline
\hline

P1 & No Pre-claimed Custom Permission
& All
& \textbf{if} \blue{$Id_{a} \neq Id_{v}$} $\land$ \blue{$\exists(PermAttr_{v} \notin SysPerms)$} $\land$ \blue{$PermAttr_{v} = PermAttr_{a}$}: \textbf{deny}
& \cha
\tabularnewline \hline

P2 & No By-default Exported Provider
& P
& \textbf{if} \blue{$Id_{a} \neq Id_{v}$} $\land$ \blue{$\neg ExportedAttr$}: \textbf{deny}
& \ling
\tabularnewline \hline

P3 & Alerting Explicitly Exported Provider
& P
& \textbf{if} \blue{$Id_{a} \neq Id_{v}$} $\land$ \blue{$ExportedAttr = true$}: \textbf{alert}
& \cha
\tabularnewline \hline

\multirow{2}{*}{P4} & No By-default Exported Component
& \multirow{2}{*}{A,S,R}
& \multirow{2}{*}{\textbf{if} \blue{
  $Id_{a} \neq Id_{v}$} $\land$ \blue{$\neg ExportedAttr$} $\land$ \blue{$ActionAttr \notin SysActions$
  }: \textbf{alert}}
& \multirow{2}{*}{\gou}
\tabularnewline
& for Custom Intent Action & & & \tabularnewline
\hline

P5 & Checking System-only Broadcasts
& R 
& \textbf{if} \blue{$Id_{a} \neq Id_{v}$} $\land$ \blue{$\exists (ActionAttr \in SysActions)$} $\land$ \blue{$InputAction \neq ActionAttr$}: \textbf{deny}
& \gou
\tabularnewline \hline

P6 & Filtering Sql Injection for Provider
& P
%$InputPara \supseteq AttackStr$
& \textbf{if} \blue{$Id_{a} \neq Id_{v}$} $\land$ \blue{$\exists (AttackStr \in InputPara)$}: \textbf{deny}
& \cha
\tabularnewline \hline

\end{tabu}
\begin{tablenotes}
\item[\dag] This column lists which components this policy is applicable for. The five symbols are explained as follows.\\
  All: all four components; A: \texttt{Activity}; S: \texttt{Service}; R: \texttt{Receiver}; P: \texttt{Provider}.
\end{tablenotes}
\end{threeparttable}
}
\label{tab:macpolicy}
%\vspace{-2ex}
\end{table*}


We manage to devise mandatory access control (MAC) policies to stop common component hijacking issues.
These issues arise because of system flaws or developer mistakes.
We study their root causes and design the corresponding MAC policies for \entryAC to enforce.
Table~\ref{tab:macpolicy} lists six representative MAC policies (P1 to P6) we have designed.
From a high-level view, policies P1 to P3 patch the system weaknesses, P4 and P5 mitigate common developer mistakes, and P6 filters a common attack.


A common point among all six policies is that we treat the IPC requests initiated from the same app or developer trusted.
That is, only an external IPC request from a third-party app will be checked.
This is denoted by $Id_{a} \neq Id_{v}$, as mentioned in \mysec\ref{sec:primitive}.
However, an experienced adversary may bypass this policy by detouring IPC requests first to another component in the victim app.
We propose to mitigate this problem by adding a flag during each IPC relay so that \name can infer the origin of an IPC call chain.
For example, we can add one line of code, \texttt{intent.putExtra(`seclibflag', `outside')}, into each \sinkAC instrumentation that contains IPC call functions.


The policy \textbf{P1} is derived from a system flaw~\cite{CustomPermission} that an attack app who installed earlier can pre-claim a custom permission in the victim app, such as setting its permission level from \texttt{signature} to \texttt{normal}.
Consequently, the attack app can hijack any component that was originally protected with \texttt{signature}-level permissions.
Based on this root cause, our policy first determines whether there is a custom permission defined in the callee component, i.e., $\exists(PermAttr_{v} \notin SysPerms)$.
If there is a such custom permission, we further check whether or not it has been pre-claimed by the caller app, i.e., $PermAttr_{v} = PermAttr_{a}$.
If yes, we deny the request to prevent a component hijacking attack.


The policy \textbf{P2} and \textbf{P3} aim to mitigate the gap that components could be by default exported by system whereas developers may not be aware of that.
Specifically, components that define Intent Filters are implicitly exported~\cite{Intent} even if they do not claim the ``exported'' attribute.
Furthermore, \texttt{Provider} components are automatically exported unless developers explicitly assign ``false'' to the ``exported'' attribute.
This by-default rule led to thousands of vulnerable \texttt{Provider} components~\cite{ContentScope13}.
Although Google later revised this rule since Android 4.2, it still requires developers to manually update apps' SDK attributes to a safe version.
According to a very recent study~\cite{TargetFragmentation16}, there are still many by-exported \texttt{Provider} components.


To protect by-default exported component from hijacking, policy \textbf{P2} and \textbf{P3} first determine whether there exists the ``exported'' attribute.
For \texttt{Provider}, we can deny the IPC request if there is no ``exported'' attribute, in order to mimic the current system rule.
For other components, we further check what kinds of \texttt{Intent} actions are registered.
Only for those custom actions ($ActionAttr \notin SysActions$), the corresponding IPC requests will be denied.
Additionally, we will provide a debug mode with user interfaces, to help developers resolve the potential (but less likely) conflict between their original intentions and our policies.


Following P3, we further propose the policy \textbf{P4} to handle the case of system actions.
In particular, a component listening to system-only broadcasts is hijack-able if it does not check the incoming \texttt{Intent} action explicitly in the code.
A prior work \cite{ECVDetector14} showed that there are around 150 system-only broadcasts on Android.
To prevent component hijacking due to missed action checks, P4 automatically checks the input action against the system-only action claimed in manifest, i.e., $\exists (ActionAttr \in SysAction)$ $\land$ $InputAction \neq ActionAttr$.


The policy \textbf{P5} aims to mitigate the denial-of-service hijacking due to missed null checks on IPC input.
This is a common mistake that affected a large portion of Android apps, according to a previous empirical study~\cite{Study11}.
To stop such hijacking, we record the app crash times corresponding to each caller app.
And if it has exceeded the threshold value (e.g., 3 times), \name then denies the request. 
Moreover, we can consider only the recent crashes to avoid over-checking.


Finally, we propose the policy \textbf{P6} to filter SQL injection for \texttt{Provider}.
As demonstrated in~\cite{ContentScope13}, an attack app can hijack a \texttt{Provider} component to inject malicious SQL statements.
For example, the adversary sets the \texttt{projection} parameter of the \texttt{query} function as a special phase ``\texttt{* from private\_table;}''.
Since these special inputs are usually different from normal queries, we thus can use keyword-based filtering (such as the keyword ``\texttt{;}'') to stop them. 

